Capturing Detailed Deformations of Moving Human Bodies

We present a new method to capture detailed human motion, sampling more than 1000 unique points on the body. Our method outputs highly accurate 4D (spatio-temporal) point coordinates and, crucially, automatically assigns a unique label to each of the points. The locations and unique labels of the points are inferred from individual 2D input images only, without relying on temporal tracking or any human body shape or skeletal kinematics models. Therefore, our captured point trajectories contain all of the details from the input images, including motion due to breathing, muscle contractions and flesh deformation, and are well suited to be used as training data to fit advanced models of the human body and its motion. The key idea behind our system is a new type of motion capture suit which contains a special pattern with checkerboard-like corners and two-letter codes. The images from our multi-camera system are processed by a sequence of neural networks which are trained to localize the corners and recognize the codes, while being robust to suit stretching and self-occlusions of the body. Our system relies only on standard RGB or monochrome sensors and fully passive lighting and the passive suit, making our method easy to replicate, deploy and use. Our experiments demonstrate highly accurate captures of a wide variety of human poses, including challenging motions such as yoga, gymnastics, or rolling on the ground.

==> Backups.tex <==
When precise measurements are needed, prior work relies on either 1) reflective markers attached to a motion capture suit or glued to the skin \cite{park2006capturing}, or 2) painting colored patterns on the skin \cite{bogo2017dynamic}.

Those are the strong points that I want to put in the introduction:
\begin{itemize}
    \item Uniquely label the markers, only relying on local features, which allows us to capture more challenging poses.
    \item Directly get 4D data without relying on temporal tracking, human body shape or kinematics model
    \item Can be directly used as ground truth data
    \item Robust despite large deformations of human skin and self-occlusion
    \item Allow parallel processing
    \item Rely on standard RGB or monochrome sensors
    \item passive light only
\end{itemize}

This is how I plan to fulfill the rest of the Introduction:

\paragraph{Part 1,} downsides of two ways to get accurate measurements (reflective markers, painting colored patterns)
\begin{itemize}
    \item \textbf{Problem of reflective markers}: marker labeling is hard, which limits the total number of markers that can be used.
    \item \textbf{Problem of painting colored patterns}: relies on the texture, which have to be generated from the geometric registration. Limited volume of capture. All those limited the variety of poses that can be captured. Besides, the price of the system is prohibitive.
\end{itemize}

\paragraph{Part 2}Our solution:
\begin{itemize}
    \item Our solution is, putting fiducial markers on the subject's body, using a special capture suit.
    \item Unlike painting colored patterns directly on skin, the suit allows us to print a sophisticatedly designed high-resolution image on it, which includes more than one thousand fiducial markers enabling both accurate localization, and inference of unique labels which is temporally invariant for each marker. The suit naturally moves along with the body, thus the markers represent temporally consistent locations on the body.
    \item The  localization and labelling of fiducial markers, which is just a small patch on the suit, only relies on the local suit feature, thus is robust despite large deformations of human skin and self-occlusion.
    \item Consequently, we are able to capture a more variety of motions, including challenging motions, like yoga poses with significant self occlusions, and like rolling on the ground which requires large capture volume.
    \item By reconstructing those markers, we directly obtain the 4D data of human motion with a unique label for each marker, without requiring registration of template mesh, prior human body shape or kinematics model. Instead, our trajectories can be used as ground truth data.
    \item The independence between frames, also allows us to process them in parallel.
    \item Low cost of only relying on standard RGB or monochrome sensors 
\end{itemize}

Then I will talk about our evaluation method and discuss our results.

==> Old_03_FiducialMarkerCaptureSystem.tex <==
\section{Fiducial Marker Capture System}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figs/SuitComparison.pdf}
    \caption{(a) Classical motion capture suit and marker. (b) The design of our motion capture suit with fiducial markers. (c) The fiducial marker is consisted of checkerboard-like corners and codes.}
    \label{fig:SuitDesign}
\end{figure}
An important innovative aspect of our method is a suit with specially designed texture, containing more than 1400 uniquely identifiable markers.  The marker is a combination of two key elements  (Fig. \ref{fig:SuitDesign}c): 1)
\textit{corners} between the black-and-white squares that can be localized with sub-pixel accuracy, similar to classical computer vision calibration boards, and 2)
unique two-letter \textit{codes} written in the white squares that enable unique corner labeling. We use only characters that have unique upright orientation specifically "1234567ABCDEFGJKLMPQRTUVY", intentionally avoiding characters such as "0" and also "9" that could be confused with rotated "6".
% The cost to make such a suit is around \$50, everyone can make the suit and
% build up the capture system at a relatively low cost.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figs/SystemIllustration.pdf}
    \caption{(a) A photo of our 16 camera setup. (b) The cameras form a circle surrounding the capture volume, the ground is defined as the XY-plane of our coordinate system.}
    \label{fig:System}
\end{figure}
Our multicamera setup contains 16 standard (RGB) cameras arranged into a circle surrounding the capture volume (Fig. \ref{fig:System}b). Each camera captures 4000$\times$2160 images at 30 FPS in RAW format. The camera shutters are synchronized via genlock with error on the order of microseconds, which is negligible.

\subsection{Marker Localization and Labeling}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figs/CNNPipeline2.pdf}
    \caption{Marker localization and labeling pipeline: (a) a \textit{Corner Detector} ConvNet detects our suit corners; (b) visualization of a subset of quad proposals that are generated by connecting the corners detected in the previous step; (c) homography undistortion of the quads, generating all four possible orientations; (d) a \textit{Rejector} ConvNet is a binary classifier accepting only correctly connected corners with valid upright orientation; (e) a \textit{Recognizer} ConvNet converts the accepted codes to text.}
    \label{fig:CNNPipeline}
\end{figure*}
We propose a multi-stage approach to localize and label the corners visible in our images, see Fig. \ref{fig:CNNPipeline}. Our method utilizes the two elements on the suit -- we localize the corners, and then try to read the codes linked to the corners.  
The convolutional neural networks (CNN) are perfectly suited for automating the task of localizing and labeling markers using those elements.

The first step of the pipeline is a \textit{Corner Detector} ConvNet which detects all checkerboard-like corners and localizes them with sub-pixel accuracy (Fig. \ref{fig:CNNPipeline}a). This network is discussed in \TODO{Section XXX}.

\TODO{start rewriting here}
The next step is to read the codes and find their relation to the corners, which will uniquely label the detected corners. As shown in Fig. \ref{fig:teaster}a, the deformation of the code including stretching, tilting, and rotation can be quite significant due to the motion of the body. All those add to the difficulty to recognize codes.
A well explored approach \cite{long2020scene} to deal with those spatial deformation is to concatenate multiple stages: detect the region proposals (text boxes) in the wild, correct its orientation and distortion, then feed the corrected image to RecogNet. We also take multiple stages to maximize the reliability of the labelling result. The suit are designed to  provides a way to generate text box by utilizing the checkerboard-like structure of the markers.
% Luckily, we already got the corners detected, which we perform a key role in the following step of correcting the spatial deformation.

On our suit, all the codes are in white squares whose 4 corners are exactly the corners we detected in the first step. Thus practically we generate the region proposals by enumerating the 4-combinations of all the corners. We name those regions "Quad proposals" (Fig. \ref{fig:CNNPipeline}b), we unwarp those quads by mapping its four corners to a regular square by computing a homography deformation (Fig. \ref{fig:CNNPipeline}c), and cropping it to be used as the input to the CNN classifier.

This gives us several advantages: 
\begin {enumerate*} [label=\itshape\alph*\upshape)]
\item Since the square is only a small patch on the suit, practically the homography can counteract most of the spatial transformation that is added to the codes (e.g., Fig.\ref{fig:CNNPipeline}c), which significantly improved the robustness of labelling process. 
\item Since the quads are generated by corners, we naturally have the relation between the corners and the codes.
\item The CNN classifier can act like a quality controller, rejecting those white squares whose corners are not detected correctly, which adds to the robustness of the corner localizing procedure. 
% \TODO{Add a figure to illustrate this. What kind of quads should be accepted.}
\end {enumerate*} 
\TODO{end rewriting here; these paragraphs are poorly structured. Please explain the pipeline first (quad proposals etc.) and then discuss why did we design it the way we did. Don't mix up suit design with pipeline description and related work. Remember, the reviewers have never seen our pipeline before, they don't know how it works, you've to explain it to them first and then argue why we think this is a good choice. In the current text it's all mixed up together and it'd be very hard for the reviewers to understand how our pipeline actually works.}

\subsubsection{Corner Detector}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figs/CornerDet.pdf}
    \caption{The illustration of our CornerdetNet. (a) The input image is divided into a grid, size of each block is $8\times 8$\TODO{you need to talk about the 8x8 active windows inside each patch in the main text of the paper, not just in the caption. Captions are optional to read.}. (b) The image is cropped into patches around each $8\times 8$ block plus a 6 pixels wide margin (lighter green), making size of each patch $20\times 20$\TODO{this illustration would be much clearer with a real URSA image, as opposed to these lighter/darker green diagrams}. Note that the margin overlaps with neighboring blocks. \TODO{again, move this to the main text and explain why do we have this overlap}
    % The region with lighter green color is the margin area, which overlaps with other patch's darker green region. 
    (c) The architecture of our \textit{Corner Detector} network. (d) CornerdetNet outputs 3 numbers. First number is the probability that the patch has one valid corner in its central $8\times 8$ window. Last two numbers are the normalized coordinate of the corner. \TODO{There is no point in repeating what already is in the main text of the paper.} In the examples, only the third patch has a valid corner within the central $8\times 8$ window, thus the last two number is only meaningful for the third patch. Note that even though there is a corner in the margin region for the second region, it should still output 0 for the first number\TODO{This is what you want to keep in the caption -- you're explaining what the reviewers see in the figure. Please also explain why it should output 0 in this case.}.
    }
    \label{fig:CornerDetector}
\end{figure*}
The corners on our suit are approximately uniformly distributed; a small image patch is enough to detect and localize a corner. Therefore, we start by dividing our input image into a series of overlapping patches\TODO{this needs a small figure explaining the overlap} and then feed these 20x20 patches to our \textit{Corner Detector} ConvNet. The \textit{Corner Detector} processes all patches independently and 1) detects whether a corner is present or not (binary classifier) and 2) if a corner is present, outputs its subpixel coordinates relative to the 20x20 patch.

\TODO{move this to Related Work or delete it:
tries to identify and localize one corner from each patch. This naturally controls the sparsity of the corners and allows us have floating number level of accuracy for the corner location in comparison to the heat map based method \cite{detone2018superpoint}, where the accuracy is limited by how fine the pixels are divided into subpixels.}

Our CornerdetNet takes a $20\times20 \times 1$ image as input, where 1 is the number of channels. We convert the image to grayscale image using our white balance calibration, to reduce influence of Bayer patterns to localization accuracy. \TODO{Add more elaboration if white balancing.} \TODO{This should have been explained first, this is the first step in the pipeline -- please reorganize the text accordingly. Illustrate the de-Bayering with a figure and explain that we do this so we don't lose any precision by standard RGB demosaicing.} Our CNN corner detector has 2 convolutional layers with kernel size $5\times 5$ and 4 fully connected layers, the first conv layer is followed by a $2\times 2$ max pooling layer \TODO{what's the point of explaining part of the ConvNet architecture in text? refer to the figure instead}. The output of \textit{Corner Detector} are three  floating-point numbers. The first one is a logit of a binary classifier predicting whether a corner is present or not and the other 2 are normalized coordinates of the corner relative to the patch. 
\TODO{delete this, replace by reference to papers that proposed this before, this is not new: 
%
The training loss is:
$$
\mathcal{L}_c(p^*, p;  \mathbf{c}^*, \mathbf{c}) = \lambda_{p} L_p(p^*, p) + \lambda_{c} P_c||\mathbf{c}-\mathbf{c}^*||^2.
$$
Where the $p^*$ and ${c}^*$ represents the prediction, $p$ and ${c}$ represents the ground truth, and $L_p(p^*, p)$ represents cross entropy:
$$
 \mathcal{L}_p(p^*, p) =  -p ln(p^*) -(1 - p) ln(1 - p^*)
$$}

\TODO{you're missing discussion why the patches are overlapping (so we don't miss any corners in the 20x20 patches), what is the padding, I think it was 8x8 + 6 pixel margins, that after the Corner Detector we do postprocessing via clustering to remove repeated detections. Discuss the assumptions we are making: that no corners will be closer than 8 pixels. Please refer to the code for details, my memory is hazy and what I wrote above may not be accurate.}

\subsubsection{Quad Proposal}
 \label{QuadProposal} 
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figs/QuadClassifiers.pdf}
    \caption{The illustration of our quad proposals and quad classifiers. (a) The quad proposals is generated from detected corners, which  potentially contain white squares with code. (b) Undistort the quads using homography that maps the quad to a regular square. We add a margin to the regular square (lighter green region), as the input  for the quad classifiers. (c) We divide the job of quad classification, and deploying two networks for them: RejectorNet and RecogNet. RejectorNet outputs the probability of the quad being a  valid white square  containing codes and with correct orientation, and RecogNet has 2 sets of 25 classes softmax output layer,  which corresponds to the 25 characters we used on the suit.
    }
    \label{fig:QuadClassifiers}
\end{figure*} \TODO{you want to start be reminding the reviewer what is the problem we're trying to solve in this stage of the pipeline, why they should bother reading about some "Quad Proposal"?}
Generally, we can detect hundreds of corners from each camera. 
We use those corners to generate region proposals\TODO{doesn't ``region proposal'' mean something else in computer vision literature?} that potentially contain codes. The ideal region proposal will be the quadrilateral made of 4 corners from one white square, which contains the two-letter code, because by mapping its four corners to a regular square using a homography deformation we can best undistort the warpping of the code, like the orange and yellow quadrilaterals in Fig\ref{fig:CNNPipeline}b. We call those quadrilateral-shaped region proposals "quad proposals".

However, it would be unwise to generate possible quad proposals from all possible 4-combinations of corners. Practically, we filter out a major part of the bad combinations by their shapes. To begin with, we iterate over all the corners, and for each corner, we select other corners within certain distance to form combinations of 4 corners as candidates of quad proposal. This ensures no corners that are too far away can form into a quad. When generating those candidates, we also make sure the quads are unique, clock-wise oriented and not self-occluded. Then we further control the area, length of edge, minimum angles, average intensity and standard deviation of the pixel of those candidate quads, to make sure no blank or weirdly shaped quads gets to the quad classifier. This step will filter out a major part of the bad quads, leaving the rest for the quad classifiers. Note that we do not know the correct orientation of those quads yet, i.e., we do not know which corner should be the top left corner. Thus we use all 4 possible orientation for every quad proposal, and leave the classifier with the job to determine the right orientation.

\subsubsection{Rejector and Recognizer}
% We apply a unwrapping to format the input for quad classifiers. 
For each quad proposal, we use a homography to map the quad to a regular square. 
The homography can counteract most of the spatial transformation added to the code when the quad represents a white square.
The homography is computed by mapping the quad's 4 corners to a regular square's 4 corners. We add a margin to the regular square, to give the classifier a better sight of the code and also allow it to see the quality of the corners (Fig. \ref{fig:QuadClassifiers}b). For each quad proposal, we can have 4 different possible homographies, each one of them maps one of the quad's corner to the top left corner of the regular square. The size of regular square is $64\times 64$, and the width of the margin is 20 pixels. Thus the input images to classifier are of size $104\times 104$.

The unwarpped quads then go through 2 quad classifiers: one determine whether it is a valid quad, which we call "RejectorNet"; another tells us the code that is written in the white square, which we call "RecogNet". It is possible to combine those 2 network as one, but we choose not to. The reason we separate them is, if combined, we need to train them using the same data set. However, we have different expectations for those classifiers. For RejectorNet, we want it to control the quality of the quad, i.e., it should not allow any quad that is too blurry or wrinkled to go to RecogNet, it is also responsible of detecting the errors made by CornerdetNet (Fig. \ref{fig:QuadClassifiersData}f). 
% In other word, we want it to be conservative, not letting the low quality data through. Nevertheless, for RecogNet, since the data we feed to it is already be reckoned as a valid quad, we really want it to try its best to recognize the code despite its blur or distortion. In other word, we want RecogNet to be "aggressive". 
In other word, we make RejectorNet conservative by disallowing any low quality quads to be passed as inputs to RecogNet. RecogNet works as a quality controller of the whole pipeline, filtering out mistakes made by previous steps. On the other hand, we make RecogNet aggressive by training it to read the codes of even the low quality quads, since its input is supposed to be a valid quad.
% From our observation, training the data with slightly harder data can result in worse performance on the training set, but better performance on the validation set. 
For these reasons, we separate the two processes the two process and train RecogNet with harder data, by applying stronger data augmentation and using more various synthetic data (Fig. \ref{fig:QuadClassifiersData}g).

RejectorNet and RecogNet have similar network structure, only the output layers are different. Both RejectorNet and RecogNet have 4 convolutional layers with kernel size of 5, each followed by a $2\times 2$ max pooling layer.  RejectorNet has 4 fully connected layers, and a logistic output layer tells the probability that input is a valid white square with readable code in it. RecogNet's conv layers are connected to 2 parallel sets of 4 fully connected layers, each with a 25 classes softmax output layer, which corresponds to the 25 characters we used on the suit, predicting the 2 characters that is written in the square. We use standard cross entropy loss to train those classifiers.

\subsection{Uniquely Label Corners and Triangulation}
After the aforementioned processing, we can uniquely label each corner. Because every code on the suit is unique and and its upright orientation is also uniquely defined, technically, it is enough to uniquely label its 4 corners once a quad is recognized. In fact, for most of the corners on the suit, it has 2 adjacent codes, which will work as a redundancy check to increase the robustness of the labelling procedure. We assign a unique ID number to every corner on the suit. We use $I_c$ to denote the unique ID number of corner $\mathbf{c}$. Note that $I_c$ only depends on the suit, and is invariant with respect to time. For our suit, the range of $I_c$ is 0 to 1486.

After we figure out $I_c$ for each detected corner, we have the correspondence between corners in different cameras in the same frame (spatial), and correspondence between corners in different frames, without need for sequential tracking (temporal).
% "Spatial correspondences" means the correspondence between corners in different cameras in the same frame, and "temporal correspondences" means correspondence between corners in different frames. The unique ID number naturally gives us those correspondences, no registration is needed.
Using the spatial correspondences, we can easily triangulate those corners by minimizing the reprojection error. Let $\mathbf{c}_i^k \in \mathbb{R}^2$ be the pixel coordinates of corner with unique ID number $i$, in camera $k \in \mathcal{C}$, $\mathcal{C}$ is the set of all the cameras. Let $\mathcal{C}_i$ be the set of cameras that see corner $i$. $f^k:\mathbb{R}^3 \to \mathbb{R}^2 $ is the projection function of camera $k$. We reconstruct corner $\mathbf{p}_i$ by minimizing the reprojection error:
\begin{equation}
\mathbf{p}_i = \underset{\mathbf{p}_i\in \mathbb{R}^3}{\arg\min} \sum_{k\in \mathcal{C}_i } ||  f^k(\mathbf{p}_i)-\mathbf{c}_i^k||^2_2 
\end{equation}
This is a non-linear least square optimization problem. Practically we initialize $\mathbf{p}_i$ using Linear-LS method \cite{hartley1997triangulation}, then optimize it using non-linear least square solver. We remove the reconstructed corners with average reprojection error more than 1.5. Fig. \ref{fig:Reprojection}, illustrated the distribution of reprojection errors per camera in 10,000 frames including various types of motions. $99\%$ of the marker points has an average reprojection errors less than $0.31$ pixel. The large reprojection errors most come from the wrong Recognition results, which set up wrong matches between corners in different cameras. This can happen to a corner with only one adjacent code recognized, in which case the redundancy check does not work. However, those cases generally results in a large reprojection error, and can be easily filtered out by setting threshold to the  reprojection errors. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figs/Reprojection.png}
    \caption{The histogram of reprojection errors (in pixel)  per camera for all the reconstructed points in 10000 frames, note that the X-axis and Y-axis are both in log scale. }
    \label{fig:Reprojection}
\end{figure}


